Analysis and mitigation of pulse-pile-up tail artifacts in warm-plasma pulse-height X-ray spectra

Pulse pile-up in pulse-height energy analyzers increases when the incident rate of pulses increases relative to the inverse of the dead time per pulse of the detection system. Changes in the observed energy distributions with incident rate and detector-electronics-formed pulse shape then occur. We focus on weak high energy tails in X-ray spectra, important for measurements on partially ionized, warm, pure-hydrogen plasma. A first-principles two-photon pulse-pile-up model is derived specific to trapezoidal-shaped pulses; quantitative agreement is found between the measurements and the model predictions. The modeling is then used to diagnose pulse-pile-up tail artifacts and mitigate them in relatively low count-rate spectra.

==> bibliography.tex <==
@misc{radiology,
  title = {{Pulse-Height Spectrometry}},
  publisher={Radiology Key},
  howpublished = {\url{https://radiologykey.com/pulse-height-spectrometry}},
  note = {Accessed: December 10, 2020}
}

@book{globalsino,
	author="Yougui Liao",
	title="Practical Electron Microscopy and Database",
	year="2006",
	publisher="Globalsino",
	pages="2532",
	note={\url{https://www.globalsino.com/EM/page2532.html}}
}

@book{spieler,
	author="Helmuth Spieler",
	title="Pulse Processing and Analysis",
	year="2002",
	publisher="IEEE NPSS Short Course",
	pages="41"
}

@misc{data,
    title={http://arks.princeton.edu/ark:/88435/dsp01x920g025r},
}



@article{Glasser,
author = {A.H. Glasser and Cohen, S.A. },
title = {Ion and electron acceleration in the field-reversed configuration with an odd-parity rotating magnetic field},
journal = {Phys. Plasmas},
volume = {9},
number = {5},
pages = {2093-2102},
year = {2002},
doi = {10.1063/1.1459456},
URL = {https://doi.org/10.1063/1.1459456},
eprint = {https://doi.org/10.1063/1.1459456}
}

@article{crystal,
	author = {Beiersdorfer,P.  and von Goeler,S.  and Bitter,M.  and Hill,K.W.  and Hulse,R.A.  and Walling,R.S. },
	title = {High‐resolution bent‐crystal spectrometer for the ultrasoft x‐ray region},
	journal = {Review of Scientific Instruments},
	volume = {60},
	number = {5},
	pages = {895-906},
	year = {1989},
	doi = {10.1063/1.1140341},
	URL = {https://doi.org/10.1063/1.1140341},
	eprint = {https://doi.org/10.1063/1.1140341}
}

 @misc{amptek, 
 	title="{X-123SDD Complete X-Ray Spectrometer with Silicon Drift Detector (SDD) – Amptek – X-Ray Detectors and Electronics}", 
 	howpublished={{https://amptek.com/products/x-ray-detectors/sdd-x-ray-detectors-for-xrf/x-123sdd-complete-x-ray-spectrometer-with-silicon-drift-detector-sdd}},
 	note={Accessed: December 12, 2020}
}

@article{charles,
	author = {Swanson,C.  and Jandovitz,P.  and Cohen, S.A. },
	title = "{Using Poisson-regularized inversion of Bremsstrahlung emission to extract full electron energy distribution functions from x-ray pulse-height detector data}",
	journal = {AIP Advances},
	volume = {8},
	number = {2},
	pages = {025222},
	year = {2018},
	doi = {10.1063/1.5019572},
	URL = {https://doi.org/10.1063/1.5019572},
	eprint = {https://doi.org/10.1063/1.5019572}
}

@misc{myscope, 
	title={{X-ray detection by EDS}},
	publisher={MyScope},
	howpublished={\url{https://myscope.training/legacy/analysis/eds/xraydetection/}},
	note= {December 10, 2020}
}

@article{datlowe,
	title = {The role of the waveform in pulse pile-up},
	journal = {Nuclear Instruments and Methods},
	volume = {145},
	number = {2},
	pages = {365-378},
	year = {1977},
	issn = {0029-554X},
	doi = {https://doi.org/10.1016/0029-554X(77)90435-9},
	url = {https://www.sciencedirect.com/science/article/pii/0029554X77904359},
	author = {Dayton W. Datlowe}
}

@article{guo,
	title = "{The Monte Carlo approach MCPUT for correcting pile-up distorted pulse-height spectra}",
	journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
	volume = {531},
	number = {3},
	pages = {520-529},
	year = {2004},
	issn = {0168-9002},
	doi = {https://doi.org/10.1016/j.nima.2004.05.089},
	url = {https://www.sciencedirect.com/science/article/pii/S016890020401112X},
	author = {Weijun Guo and Sang Hoon Lee and Robin P. Gardner},
}

@article{taguchi,
	author = {Taguchi, Katsuyuki and Frey, Eric and Wang, Xiaolan and Iwanczyk, Jan and Barber, William},
	year = {2010},
	month = {08},
	pages = {3957-69},
	title = {An analytical model of the effects of pulse pileup on the energy spectrum recorded by energy resolved photon counting x-ray detectors},
	volume = {37},
	journal = {Medical physics},
	doi = {10.1117/12.843753}
}

@article{Wang,
  	author={J. {Wang} and L. {Chen} and M. {Persson} and P.L. {Rajbhandary} and P. {Kandlakunta} and G. {Carini} and R. {Fahrig}},
    journal={IEEE Transactions on Nuclear Science}, 
    title={Pulse Pileup Analysis for a Double-Sided Silicon Strip Detector Using Variable Pulse Shapes},
    year={2019},
    volume={66},
    number={6},
    pages={960-968},
    doi={10.1109/TNS.2019.2917144}
}


@unpublished{rubin,
	author  = {T. Rubin and T. Qian},
	title   = "{Pulse pile-up correction for X-ray spectra measured by Amptek X-123 Silicon Drift Detector}",
	year    = {2020},
	note    = {unpublished}
}

@unpublished{ben, 
	author={B.M. Alessio}, 
	title={Junior Paper},
	school={Princeton University},
	year={Fall 2020},
	note={Unpublished, Princeton University}
	}

@book{redus,
	author="R. Redus",
	title="Front End Electronics for Radiation Detection and Measurement",
	year="2017",
	publisher="IEEE NPSS Short Course",
	pages="71"
}

@article{pfrc-2,
	author = {Cohen,S.A.  and Brunkhorst,C.  and Glasser,A.H.  and Landsman,A.S.  and Welch,D. },
	title = "{RF Plasma Heating in the PFRC‐2 Device: Motivation, Goals and Methods}",
	journal = {AIP Conference Proceedings},
	volume = {1406},
	number = {1},
	pages = {273-276},
	year = {2011},
	doi = {10.1063/1.3664976},
	URL = {https://aip.scitation.org/doi/abs/10.1063/1.3664976},
	eprint = {https://aip.scitation.org/doi/pdf/10.1063/1.3664976}
}
@article{PhysRevLett.98.145002,
  title = {Formation of Collisionless High-$\ensuremath{\beta}$ Plasmas by Odd-Parity Rotating Magnetic Fields},
  author = {Cohen, S.A. and Berlinger, B. and Brunkhorst, C. and Brooks, A. and Ferraro, N. and Lundberg, D.P. and Roach, A. and Glasser, A.H.},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {14},
  pages = {145002},
  numpages = {4},
  year = {2007},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.145002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.98.145002}
}

@article{Mylar,
author = {Galea, C.A.  and Swanson, C.P.S.  and Thomas, S.J. and Cohen, S.A.},
title = {Use of a Mylar filter to eliminate VUV pulse pileup in low-energy x-ray measurements},
journal = {Review of Scientific Instruments},
volume = {93},
pages = {093531},
year = {2022}
}

@article{Jandovitz,
author = {Jandovitz, P.  and Swanson, C.P.S.  and Matteucci, J.  and Oliver, R.  and Pearcy, J.  and Cohen, S.A. },
title = {Demonstration of fast-electron populations in a low-pressure, low-power, magnetized RF plasma source},
journal = {Physics of Plasmas},
volume = {25},
number = {3},
pages = {030702},
year = {2018},
doi = {10.1063/1.4998735},
URL = {https://doi.org/10.1063/1.4998735},
eprint = {https://doi.org/10.1063/1.4998735}
}

@article{Spontaneous,
author = {Swanson, C.  and Cohen, S.A.},
title = {Spontaneous multi-keV electron generation in a low-RF-power axisymmetric mirror machine},
journal = {Physics of Plasmas},
volume = {26},
number = {6},
pages = {060701},
year = {2019},
doi = {10.1063/1.5093905},

URL = { 
        https://doi.org/10.1063/1.5093905
    
},
eprint = { 
        https://doi.org/10.1063/1.5093905
    
}

}

@article{poisson-regularized,
author = {Swanson,C.  and Jandovitz,P.  and Cohen,S.A. },
title = {Using Poisson-regularized inversion of Bremsstrahlung emission to extract full electron energy distribution functions from x-ray pulse-height detector data},
journal = {AIP Advances},
volume = {8},
number = {2},
pages = {025222},
year = {2018},
doi = {10.1063/1.5019572},
URL = {https://doi.org/10.1063/1.5019572},
eprint = { https://doi.org/10.1063/1.5019572}
}




@article{ Chantler2009,
author = {Chantler,C.T. and Olsen,K. and Dragoset,R.A. and Chang,J. and Kishore,A.R.  and  Kotochigova,S.A. and Zucker,D.S.  },
title = {X-Ray Form Factor, Attenuation, and Scattering Tables},
journal = {NIST},
year = {2009},
doi = {10.18434/T4HS32},
URL = { https://www.nist.gov/pml/x-ray-form-factor-attenuation-and-scattering-tables/},
eprint = {https://doi.org/10.18434/T4HS32}
}

